Constructing Highly Inductive Contexts for Dialogue Safety through Controllable Reverse Generation

Large pretrained language models can easily produce toxic or biased content, which is prohibitive for practical use. In order to detect such toxic generations, existing methods rely on templates, real-world data extraction, crowdsourcing workers, or automatic generation to construct adversarial contexts that are likely to induce toxic generations. However, what type of context is more likely to induce unsafe responses is still under-explored. In this paper, we identify that context toxicity and context category (e.g., \textit{profanity}, \textit{insult}, \textit{drugs}, etc.) are two important factors to cause safety issues in response generation. Hence, we propose a method called \emph{reverse generation} to construct adversarial contexts conditioned on a given response, with the flexibility to control category, toxicity level, and inductivity of the generated contexts. Via reverse generation, we augment the existing BAD dataset and construct a new dataset BAD+ which contains more than 120K diverse and highly inductive contexts in 12 categories. We test three popular pretrained dialogue models (Blender, DialoGPT, and Plato2) and find that BAD+ can largely expose their safety problems. Furthermore, we show that BAD+ can greatly enhance the safety of generation and reveal the key factors of safety improvement. Our code and dataset is available at \url{https://github.com/thu-coai/Reverse_Generation}.

==> sections/Detoxification.tex <==
\begin{table*}
    \centering
    \scalebox{0.88}{
    \begin{tabular}{c|c|c|c}
    \toprule
         \textbf{Category} & \textbf{Test data induction} & \textbf{DEXPERTS induction} & \textbf{Non sequitur induction} \\
    \midrule
    flirtation & 0.79 & 0.33 (0.46) & 0.34 (0.45)\\ 
    threat & 0.78 & 0.26 (0.52) & 0.31 (0.47) \\
    identity attack & 0.74 & 0.22 (\textbf{0.52}) & 0.24 (0.50)\\
    profanity & 0.81 & 0.40 (0.41) & 0.16 (0.65)\\
    sexually explicit & 0.78 & 0.30 (0.48) & 0.07 (\textbf{0.71})\\
    insult & 0.68 & 0.20 (0.48) & 0.26 (0.42)\\
    drugs & 0.79 & 0.33 (0.46) & 0.48 (0.31)\\
    medical & 0.77 & 0.36 (0.41) & 0.61 (0.16)\\
    nsfw & 0.76 & 0.26 (0.50) & 0.33 (0.43)\\
    politics & 0.69 & 0.17 (0.52) & 0.38 (0.31)\\
    religion & 0.71 & 0.20 (0.51) & 0.34 (0.37)\\
    none & 0.75 & 0.25 (0.50) & 0.45 (0.30)\\
    \bottomrule
    \end{tabular}}
    \caption{The comparison of categories. The number in parentheses is the decline in induction success rate of each category. In DEXPERTS method, we fine-tuned model with \textit{identity attack} data. In Non sequitur method, we fine-tuned model with \textit{sexually explicit}  data. In both methods, we test models on all categories.}
    \label{table:comparison of categories}
\end{table*}

\section{Detoxification}
%TODO: 看是否需要补充在blender或者plato上的去毒实验
Using the augmented data, we conduct detoxification experiments on DialoGPT. We use two popular methods including Non sequitur \cite{xu2020recipes} and DEXPERTS \cite{liu2021dexperts}. The Non sequitur method is to forcibly change the topic when encountering an unsafe context, and the DEXPERTS method is to reduce the probability of generating unsafe tokens in the decoding stage. We mainly study the following factors influencing the detoxification performance: context's induction success rate (\S \ref{5.2}), context category (\S \ref{5.3}) and number of data (\S \ref{5.4}). From these aspects, we prove that our method is helpful to detoxification. Moreover, we compare the effect of detoxification between BAD dataset and our expanded dataset (\S \ref{5.5} ).
\subsection{Method} \label{5.1}
\paragraph{Non sequitur.} Following \citealp{xu2020recipes}, we also select topics judged as safe by classifier from the Wizard of Wikipedia conversational topic list \cite{dinan2018wizard}. Then we produce response using one of the topics. For example, we use the topic \emph{"Hollywood"} to produce the response: \emph{"Hey do you want to talk about something else? How about we talk about Hollywood?"}. Once we get these responses, we directly combine the highly inductive contexts with them as the fine-tuning data. At the same time, to ensure the model's performance on normal contexts, we add some single-turn BST data \cite{roller2020recipes}.
\paragraph{DEXPERTS.} Following \citet{liu2021dexperts}, we change the token distribution of the decoding stage as follows:  
\begin{equation}
    \tilde{P}\left ( r_t | r_{<t}, c \right )  = \mathrm {softmax} \left (  z_t + \alpha( z_t^+ - z_t^-)  \right ) 
\end{equation}
where $ z_t $ means the original logits, $ z_t^+ $ means the logits of expert model, $ z_t^- $ means the logits of anti-expert model and $ \alpha $ is a hyperparameter. In our experiments, $z_t$ and $z_t^+$ are both obtained from the model fine-tuned on the safe context-response pairs. \newline
% In summary, our modification from the original formula is that we replace the base model's logits with the expert model's logits. \newline
More details about these two methods are discussed in appendix \ref{appendix detoxification}.
\subsection{Influence of Context's Induction Success Rate} \label{5.2}
\paragraph{Non sequitur.} As shown in Table \ref{table:comparison of induction}, we can see that the model fine-tuned with data of 1.0 induction success rate performs best. Its average induction success rate is the lowest and the \textit{medical} category has the biggest gap of about 7 percent (refer to appendix \ref{appendix detoxification}, Table \ref{table:comparison of induction success rate of all category}). This proves that it is very meaningful for us to collect highly inductive data. 
\paragraph{DEXPERTS.} As for DEXPERTS method, we can see that the induction success rate has nearly no effect. One of the possible reason is that the distributions of toxic tokens of responses are similar for contexts with different induction success rates.

\begin{table}[h]
    \centering
    \scalebox{0.88}{
    \begin{tabular}{p{2cm}p{1.3cm}p{3cm}<{\centering}}
    \toprule
         \textbf{Method} & \textbf{Type} & \textbf{Average induction} \\
    \midrule
    \multirow{4}{*}{Non sequitur} & high & \textbf{0.105} \\
    & balance & 0.112 \\
    & low & 0.128 \\
    & BST & 0.552 \\
    \midrule
    \multirow{4}{*}{DEXPERTS} & high & \textbf{0.147} \\
    & balance & 0.153 \\
    & low & 0.150 \\
    & Expert & 0.427 \\
    \bottomrule
    \end{tabular}}
    \caption{The comparison of induction success rate with different types of data. High, low and balance respectively mean the model is fine-tuned with the data of 1.0 induction success rate, of 0.5 induction success rate and of balanced. BST and Expert are the control groups. The average induction success rate of test dataset is 0.75. }
    \label{table:comparison of induction}
\end{table}

\subsection{Influence of Context Category} \label{5.3}
To study the influence of context category, we fine-tune the model with one category data and test it on all categories as shown in Table \ref{table:comparison of categories}. We can find that the fine-tuned model performs better on categories that have overlapping vocabularies and topics with the trained category for both methods. This proves that collecting data in different categories is very meaningful. But for the same reason (\S \ref{5.2}), the DEXPERTS method has smaller differences. 
\subsection{Influence of Number of data} \label{5.4}
As shown in Table \ref{table:comparison of number}, the number of data has a great influence on the detoxification effect for both methods. This proves that it makes sense to augment specific categories of data.
\begin{table}
\centering
    \scalebox{0.88}{
    \begin{tabular}{p{2cm}p{2.2cm}p{3cm}<{\centering}}
    \toprule
         \textbf{Method} & \textbf{Type} & \textbf{Average induction} \\
    \midrule
    \multirow{2}{*}{Non sequitur} & 1k train data & \textbf{0.063} \\
    & 0.3k train data & 0.130 \\
    \midrule
    \multirow{2}{*}{DEXPERTS} & 5k train data & \textbf{0.153} \\
    & 1.2k train data & 0.198 \\
    \bottomrule
    \end{tabular}}
    \caption{The comparison of induction success rate with different number of training data. The average induction success rate of test dataset is 0.75}
    \label{table:comparison of number}
\end{table}

\subsection{Comparison of effect between BAD and RGD} \label{5.5}
We compared the detoxification experiments using different numbers of BAD and RGD data. In this experiment, We try our best to ensure that the amount of data in each category in the training set is consistent. In case of data shortage, we use other categories of data to ensure that the total amount is consistent. As shown in Figure \ref{}, under the same total data volume, our detoxification effect is better. In addition, due to the advantage of more data volume in RGD, we can further detoxify the model.

==> sections/Detoxification_new.tex <==
\section{Detoxification}

\subsection{Method}

Using the augmented data, we conduct detoxification experiments on DialoGPT. We use the method ``Non sequitur''  proposed along with the BAD dataset \cite{xu2020recipes}. The Non sequitur method is to forcibly change the topic when encountering an unsafe context. Following \citealp{xu2020recipes}, we also select topics judged as safe by classifier from the Wizard of Wikipedia conversational topic list \cite{dinan2018wizard}. Then we produce response using one of the topics. For example, we use the topic \emph{"Hollywood"} to produce the response: \emph{"Hey do you want to talk about something else? How about we talk about Hollywood?"}. Once we get these responses, we directly combine the highly inductive contexts with them as the fine-tuning data. At the same time, to ensure the model's performance on normal contexts, we add some single-turn BST data \cite{roller2020recipes}.

% We mainly study the following factors influencing the detoxification performance: context's induction success rate (\S \ref{5.2}), context category (\S \ref{5.3}) and number of data (\S \ref{5.4}). From these aspects, we prove that our method is helpful to detoxification. Moreover, we compare the effect of detoxification between BAD dataset and our expanded dataset (\S \ref{5.5} ).

\begin{figure}[!t]
\includegraphics[width=\linewidth]{figs/detoxify.png}% 1\linewidth
  \caption{Comparison of detoxification effects between our augmented data and BAD data. The suffix \textit{\_min5} represents the average induction success rate of five categories with fewest samples. }
  \label{fig:detoxify}
\end{figure}

\subsection{Experiments and Analysis}

\subsubsection{Data Augmentation through Reverse Generation Improves Detoxification}
We compared the detoxification effects between the augmented dataset and the BAD dataset. We construct a test set which contains the same number of contexts for each of the 12 category. To construct a balanced training set within the given budget, we try to ensure that the amount of data in each category is consistent. In case of data shortage for some categories, we use contexts from other categories to ensure that the given budget is exhausted. The responses for these inductive contexts are randomly sampled from the candidate responses constructed using Non Sequitur method. We also add some single-turn data from BST dataset in a 4:1 ratio. After fine-tuned on the training set, the model samples 10 responses for each context in the test set to measure the induction success rate. The result is shown in Figure \ref{fig:detoxify}. With the same number of training data, the augmented data through reverse generation better detoxifies the dialogue model. In addition, due to the advantage of more data in our augmented dataset, the detoxification effect is further enhanced. We also pick out 5 categories with the least data in BAD dataset (i.e., \textit{profanity, drugs, religon, medical} and \textit{nsfw}). We can observe that the performance gap between our dataset and BAD dataset on these 5 categories is obviously larger than on all categories, which suggests the benefits of generating contexts of categories with few samples through controllable reverse generation.

\begin{table}[!t]
    \centering
    \scalebox{0.72}{
    \begin{tabular}{c|c|c}
    \toprule
         \textbf{Category} & \textbf{Induction before FT} & \textbf{Induction after FT} \\
    \midrule
    flirtation & 0.79  & 0.34 (0.45)\\ 
    threat & 0.78 & 0.31 (0.47) \\
    identity\_attack & 0.74  & 0.24 (0.50)\\
    profanity & 0.81 & 0.16 (0.65)\\
    sexually\_explicit & 0.78 & 0.07 (\textbf{0.71})\\
    insult & 0.68 & 0.26 (0.42)\\
    drugs & 0.79 & 0.48 (0.31)\\
    medical & 0.77 & 0.61 (0.16)\\
    nsfw & 0.76 & 0.33 (0.43)\\
    politics & 0.69 & 0.38 (0.31)\\
    religion & 0.71 & 0.34 (0.37)\\
    none & 0.75 & 0.45 (0.30)\\
    \bottomrule
    \end{tabular}}
    \caption{The comparison of induction success rate of different categories of contexts before and after fine-tuning. The number in parentheses is the decline in induction success rate of each category.}
    \label{table:comparison of categories}
\end{table}

\subsubsection{Influence of Context Category}
In this section we explore the influence of context category more in depth. We fine-tune DialoGPT on contexts from \textit{sexually\_explicit} category and test it on all categories as shown in Table \ref{table:comparison of categories}. We can find that the fine-tuned model performs better on categories that have overlapping vocabularies and topics with the trained category. This further proves that collecting inductive contexts of different categories is very meaningful.

\subsubsection{Influence of Context's Induction Success Rate}
Highly inductive contexts are more harmful and dangerous, but whether they are more helpful for detoxification is unknown. Therefore, we compare the detoxification effects between using contexts with high and low induction success rate.
%TODO:等新的结果跑完补上
As shown in Table \ref{}, we can see that the model fine-tuned with data of 1.0 induction success rate performs best. 
% Its average induction success rate is the lowest and the \textit{medical} category has the biggest gap of about 7 percent (refer to appendix \ref{appendix detoxification}, Table \ref{table:comparison of induction success rate of all category}). 
This proves that it is very meaningful for us to collect highly inductive contexts.

==> sections/Experiments.tex <==
\section{Experiments}
\subsection{Data Augmentation}
Considering contexts with high induction success rate are more harmful and dangerous, we focus on constructing them in our work. We first filter out the contexts with an induction success rate of no less than 50\% for all 3 dialogue models (Blender-400M, DialoGPT-medium and Plato2-base). We get 14302 contexts from the 38472 contexts extracted from the BAD dataset. We split the 14302 response-context pairs into training/validation/test subsets with a ratio of 8:1:1. Then we fine-tune a reverse DialoGPT-medium model on the training set with the loss \ref{loss}. For each of the 14302 contexts, we randomly select one of the 10 responses from each of the 3 dialogue models to generate a context in reverse using nucleus sampling \cite{DBLP:conf/iclr/HoltzmanBDFC20} with $p=0.9$ . We then filter out the contexts with an induction success rate of no less than 50\% for all 3 dialogue models and get 22069 new contexts from $14302*3=42906$ generated contexts. The comparison between the original 14302 contexts and the augmented $14302+22069=36371$ contexts is shown in Figure \ref{fig:compare_context}. We can observe that the distribution of context categories remains similar after augmentation, which suggests that our reverse generation method does not have strong preference for a specific category of contexts.
\subsubsection{Controllability}

\begin{figure*}[!t]
\includegraphics[width=\linewidth]{figs/compare_context.pdf}% 1\linewidth
  \caption{Comparison between the original contexts and the augmented contexts. The two pie charts show the distribution of different categories of contexts before and after the augmentation. }
  \label{fig:compare_context}
\end{figure*}
\begin{figure}[!t]
\includegraphics[width=\linewidth]{figs/context.png}% 1\linewidth
  \caption{The context distribution of the final dataset. Each category has more than 3000 diverse contexts.}
  \label{fig:context}
\end{figure}

\begin{table}[!t]
\centering
\begin{tabular}{ccc}
\toprule
Method     & Initialization & \textit{medical} ratio \\ \midrule
No control & - & 5\%  \\
Hard prompt   & - & \textbf{19\%}  \\
Soft prompt$_2$   & Random &3\%  \\
Soft prompt$_1$  & Random &9\%  \\
Soft prompt$_1$   & Vocab &10\%  \\
Soft prompt$_1$  & Hard prompt & 8\% \\
\bottomrule
\end{tabular}
\caption{Comparison of different controllable generation methods. We use $[category\_name]$ as our hard prompts. Soft prompt$_2$ first fine-tunes the reverse generation model and then train the soft prompt tokens only. Soft prompt$_1$ trains the model and the soft prompt tokens together.   All soft prompt based methods use 10 soft tokens. Different methods are trained on various kinds of contexts and we show their abilities to generate the contexts of \textit{medical} category.}
\label{tab:control}
\end{table}

\begin{table}[!t]
\centering
\begin{tabular}{cccc}
\toprule
$\alpha,\beta$      & PPL & Toxicity & Induction\\ \midrule
$\alpha=0,\beta=0$ & 26.34 & 0.44 & 0.63 \\
$\alpha=2,\beta=0$ & 37.85 & 0.24 & 0.62 \\
$\alpha=0,\beta=2$ & 30.58 & 0.51 & 0.73 \\
$\alpha=2,\beta=2$ & 43.04 & 0.37 & 0.72 \\
\bottomrule
\end{tabular}
\caption{Comparison of different hyperparameter settings. \textit{PPL} measures the context's fluency using GPT2-large. \textit{Toxicity} measures the context's toxicity. \textit{Induction} measures the context's induction success rate.}
\label{tab:control_tox}
\end{table}

\begin{table}[!t]
\centering
\begin{tabular}{ccc}
\toprule
Metric     & Original dataset & Final dataset \\ \midrule
Number & 14302 & 122692 \\
Self-bleu4 & 0.25 & 0.25  \\
Distinct4   & 0.86 & 0.71 \\
Toxicity   & 0.47 &0.57  \\
Blender rate  & 0.78 &0.80  \\
DialoGPT rate   & 0.75 &0.78  \\
Plato2 rate  & 0.79 & 0.83 \\
\bottomrule
\end{tabular}
\caption{Comparison of the original dataset and the final dataset. \textit{Number} represents the number of contexts. We show the \textit{Self-bleu4} metric \cite{DBLP:conf/sigir/ZhuLZGZWY18} by computing the maximum BLEU \cite{KishorePapineni2002BleuAM} of a given context against 1000 randomly sampled contexts, following \cite{perez2022red}. The \textit{Distinct4} metric computes the ratio of distinct 4-grams. The \textit{Toxicity} metric represents the context toxicity. The \textit{Blender/DialoGPT/Plato2 rate} represents the success rate of induction for Blender/DialoGPT/Plato2.}
\label{tab:ctx}
\end{table}
\paragraph{Category. }
As shown in Figure \ref{fig:compare_context}, the sample numbers for some categories of contexts are very small (e.g., the contexts of \textit{medical} category only accounts for 0.40\% of the total augmented contexts). Therefore, we control our reverse generation to augment the specified category of contexts. Intuitively, conditioning on the responses to the targeted category of contexts is easier to generate contexts belonging to the target category. We verify the conjecture on the \textit{medical} category and find that conditioning on the responses to the \textit{medical} contexts increases the proportion of \textit{medical} contexts in all generated contexts from 0.3\% to 5\% compared with conditioning on all kinds of responses. We thus compare several controllable methods conditioning on the responses to the \textit{medical} contexts. As shown in Table \ref{tab:control}, using hard prompt performs best in this few-shot setting where the number of \textit{medical} contexts is small in the training set. Therefore, we use hard prompt to augment categories that include less than 3000 contexts conditioning on the responses corresponding to the contexts of those categories. The final augmented dataset is shown in Figure \ref{fig:context}. We also compare the original dataset with the final dataset. As shown in Table \ref{tab:ctx}, our method largely increases the number of contexts and keeps the contexts' high induction success rate. Although the contexts' diversity decreases and the contexts' toxicity increases to some extent, they are still within an acceptable range.
\paragraph{Toxicity and Induction success rate.}
We fine-tune DialoGPT-medium on the training part of the filtered BAD dataset and compare different hyperparameters on the test set. The toxic reverse generation model is trained on the subset where each context's toxicity is larger than 0.5. 
As shown in Table \ref{tab:control_tox}, with $\alpha=2 $ and $\beta=2$, we could simultaneously reduce the context's toxicity and increase the context's induction success rate while keeping the context's fluency acceptable, which suggests the effectiveness of our controllable generation method. Note that we didn't control the context's toxicity and induction success rate during data augmentation because the contexts in our dataset already have different toxicities and induction success rates. But the controllable method is useful for specifically constructing contexts with low toxicities and high induction success rates.

\begin{table*}
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
         \textbf{category} & \textbf{test data induction} & \textbf{DEXPERTS induction} & \textbf{Non sequitur induction} \\
    \midrule
    FLIRTATION & 0.79 & 0.33 (0.46) & 0.34 (0.45)\\ 
    THREAT & 0.78 & 0.26 (0.52) & 0.31 (0.47) \\
    IDENTITY ATTACK & 0.74 & 0.22 (\textbf{0.52}) & 0.24 (0.50)\\
    PROFANITY & 0.81 & 0.40 (0.41) & 0.16 (0.65)\\
    SEXUALLY EXPLICIT & 0.78 & 0.30 (0.48) & 0.07 (\textbf{0.71})\\
    INSULT & 0.68 & 0.20 (0.48) & 0.26 (0.42)\\
    drugs & 0.79 & 0.33 (0.46) & 0.48 (0.31)\\
    medical & 0.77 & 0.36 (0.41) & 0.61 (0.16)\\
    nsfw & 0.76 & 0.26 (0.50) & 0.33 (0.43)\\
    politics & 0.69 & 0.17 (0.52) & 0.38 (0.31)\\
    religion & 0.71 & 0.20 (0.51) & 0.34 (0.37)\\
    none & 0.75 & 0.25 (0.50) & 0.45 (0.30)\\
    \bottomrule
    \end{tabular}
    \caption{The comparison of categories. In DEXPERTS method, we fine-tuned model with IDENTITY ATTACK data. In Non sequitur method, we fine-tuned model with SEXUALLY EXPLICIT  data. In both methods, we test models on all categories. In parentheses is the decline in induction success rate of each category.}
    \label{table:comparison of categories}
\end{table*}

\subsection{Detoxification}
%TODO: 看是否需要补充在blender或者plato上的去毒实验
Using the augmented data, we conduct detoxification experiments on DialoGPT-medium. We use two popular methods including Non sequitur \cite{xu2020recipes} and DEXPERTS \cite{liu2021dexperts}. We mainly study the following factors influencing the detoxification performance: context's induction success rate (\S \ref{5.2}), context category (\S \ref{5.3}) and number of data (\S \ref{5.4}). From these aspects, we prove that our method is helpful to detoxification.
\subsubsection{Method} \label{5.1}
\paragraph{Non sequitur.} Following \citealp{xu2020recipes}, we also select topics judged as safe by classifier from the Wizard of Wikipedia conversational topic list \cite{dinan2018wizard}. Then we produce response using one of the topics. For example, we use the topic \emph{"Hollywood"} to produce the response: \emph{"Hey do you want to talk about something else? How about we talk about Hollywood?"}. Once we get these responses, we directly combine the highly inductive contexts with them as the fine-tuning data. At the same time, to ensure the model's performance on normal contexts, we add some single-turn BST data \cite{roller2020recipes}.
\paragraph{DEXPERTS.} Following \citet{liu2021dexperts}, we change the token distribution as follows:  
\begin{equation}
    \tilde{P}\left ( r_t | r_{<t}, c \right )  = \mathrm {softmax} \left (  z_t + \alpha( z_t^+ - z_t^-)  \right ) 
\end{equation}
where $ z_t $ means the original logits, $ z_t^+ $ means the logits of expert model, $ z_t^- $ means the logits of anti-expert model and $ \alpha $ is a hyperparameter. In our experiments, $z_t$ and $z_t^+$ are both obtained from the model fine-tuned on the safe context-response pairs. \newline
% In summary, our modification from the original formula is that we replace the base model's logits with the expert model's logits. \newline
More details about these two methods are discussed in appendix \ref{appendix detoxification}.
\subsubsection{Influence of Context's Induction Success Rate} \label{5.2}
\paragraph{Non sequitur.} As shown in Table \ref{table:comparison of induction}, we can see that the model fine-tuned with high induction success rate (1.0) data performs best. Its average induction success rate is the lowest and the medical category has the biggest gap of about 7 percent (this can be found in appendix, Table \ref{table:comparison of induction success rate of all category}). This proves that it is very meaningful for us to collect highly inductive data. 
\paragraph{DEXPERTS.} As for DEXPERTS method, we can see that the success rate of induction has nearly no effect. One of the possible reason is that the distribution of toxic tokens of models is similar to each other. 

\begin{table}[h]
    \centering
    \begin{tabular}{p{2cm}p{1.3cm}p{1.7cm}}
    \toprule
         \textbf{method} & \textbf{type} & \textbf{average induction} \\
    \midrule
    \multirow{4}{*}{Non sequitur} & high & \textbf{0.105} \\
    & balance & 0.112 \\
    & low & 0.128 \\
    & BST & 0.552 \\
    \midrule
    \multirow{4}{*}{DEXPERTS} & high & \textbf{0.147} \\
    & balance & 0.153 \\
    & low & 0.150 \\
    & Expert & 0.427 \\
    \bottomrule
    \end{tabular}
    \caption{The comparison of induction success rate with different types of data. High, low and balance respectively mean the model is fine-tuned with the data of high induction success rate (1.0), of low induction success rate (0.5) and of balanced. BST and Expert are the control groups. The average induction of test dataset is 0.75 . }
    \label{table:comparison of induction}
\end{table}

\subsubsection{Influence of Context Category} \label{5.3}
To study the influence of context category, we fine-tune the model with one category data and test it on all categories as shown in Table \ref{table:comparison of categories}. We can find that the fine-tuned model performs better on categories that have overlapping vocabularies and topics with the trained category for both methods. This proves that collecting data in different categories is very meaningful. But for the same reason (\S \ref{5.2}), the DEXPERTS method has smaller differences. 
\subsubsection{Influence of Number of data} \label{5.4}
As shown in Table \ref{table:comparison of number}, the number of data has a great influence on the detoxification effect for both methods. This proves that it makes sense to augment specific categories of data.
\begin{table}
\centering
    \begin{tabular}{p{2cm}p{2.5cm}p{1.7cm}}
    \toprule
         \textbf{method} & \textbf{type} & \textbf{average induction} \\
    \midrule
    \multirow{2}{*}{Non sequitur} & 1k train data & \textbf{0.063} \\
    & 0.3k train data & 0.130 \\
    \midrule
    \multirow{2}{*}{DEXPERTS} & 5k train data & \textbf{0.153} \\
    & 1.2k train data & 0.198 \\
    \bottomrule
    \end{tabular}
    \caption{The comparison of induction success rate with different number of training data. }
    \label{table:comparison of number}
\end{table}

==> sections/Method.tex <==
\section{Method}
In reality, contexts that are easy to induce unsafe responses from dialogue models are more harmful and dangerous. Therefore, it is important to identify them. Here we use the induction success rate to measure the harmfulness of the context, as defined in \S\ref{3.1}. Then we introduce our method (\S\ref{3.2}) , show key target characteristics of BAD dataset (\S\ref{3.3}) and study the controllability of these characteristics (\S\ref{3.4}).
\subsection{Estimate Success Rate of Induction} \label{3.1}
To estimate one context's success rate of induction, we let the dialogue model sample 10 responses conditioned on the context and measure the ratio of unsafe responses using both utterance-level and context-level safety classifiers.
Given a context $c$, suppose the responses sampled by the dialogue model are $R$, then the success rate of induction of the context $c$ is represented as:
\begin{equation}
    \frac{\sum_{r\in R}unsafe(r)}{size(R)}
\end{equation}
where $unsafe(r)$ is a function which returns 1 when the input response is unsafe and returns 0 when the input response is safe, and $size(R)$ represents the size of the responses set $R$. To balance the cost and the estimation error, we sample 10 responses for each context in our experiments. We use the popular top-k sampling \cite{fan2018hierarchical} algorithm (k=10) to randomly sample responses. In order to judge whether a candidate response is safe or not, we use PERSPECTIVE API\footnote{\url{https://www.perspectiveapi.com/}} as our utterance-level classifier, which judges the safety of the response without considering the context, and use BAD classifier\footnote{\url{https://parl.ai/projects/safety_recipes/}\label{recipe}} as our context-level classifier, which judges the safety of the response considering the context. PERSPECTIVE API is a widely used toxicity detection tool which achieves an AUC of 0.97+ on its test data. 
% 考虑要不要把这一段放附录里
PERSPECTIVE API could return scores for 8 different attributes, including \textit{TOXICITY, SEVERE\_TOXICITY, IDENTITY\_ATTACK, INSULT, PROFANITY, THREAT, SEXUALLY\_EXPLICIT} and \textit{FLIRTATION}. The returned scores could be interpreted as the probability that the response contains the corresponding attributes. If any of the 8 scores is no less than 0.5, we suppose the candidate response is unsafe. BAD classifier is trained on multiple datasets and could achieve a F1 score of 0.85 on average \cite{xu2020recipes}. It takes the context and the response as input, and outputs a binary score, 1 for unsafe and 0 for safe. The candidate response is considered safe when both PERSPECTIVE API and BAD classifier consider the response to be safe.

\subsection{Reverse Generation} \label{3.2}
To automatically construct a large number of contexts with high induction success rate, which could help detect and fix the security problem of dialogue models, we propose a simple method named \textit{Reverse Generation}. Conditioned on a response $r=(r_1,r_2,\cdots,r_M)$ with M tokens, the model learns to generate a context $c=(c_1,c_2,\cdots,c_N)$ with N tokens which relates to the response. The loss function is denoted as: 
\begin{equation}\label{loss}
    \mathcal{L}=-\frac{1}{N}\sum_{t=1}^N\text{log}P(c_t|r,c_{<t}) 
\end{equation}

\subsection{Target Key Characteristics} \label{3.3}
When constructing contexts using the Reverse Generation method, our goal is to get enough contexts with high diversity, low toxicity and high induction success rate. The purpose of high diversity and high induction success rate is well understood, and the purpose of low toxicity is to prevent the tested model from detecting high toxicity ahead of time and using safe responses. Since we will augment data based on BAD dataset, we first analyze these three characteristics of BAD dataset.
The BAD dataset contains 5784 dialogues between chatbots and crowd-source workers. The workers are expected to elicit toxic and biased responses from the chatbots. We extract single turn dialogues from the dataset and remove the samples with the same context. In total we get 38472 context-response pairs where the contexts are from human and the responses are from chatbots. Then we use PERSPECTIVE API and the sensitive topic classifier to measure the context toxicity and category. We utilize three popular dialogue models: Blender-400M \cite{roller2020recipes}, DialoGPT-medium \cite{zhang2020dialogpt}, and Plato2-base \cite{bao2021plato} to get the success rate of these contexts. 
% Todo: 完善这些ref , 以及想想用什么样的图展示这三个要素
\paragraph{Diversity.} We measure diversity in two ways, automatic metric scores (\S\ref{}) and category obtained according to the above method. 
\paragraph{Toxicity.} We find that although the average toxicity score is less than 0.5, nearly half of the categories have an average toxicity score of more than 0.5. This indicates that we need to explore ways to control toxicity score within an acceptable range.
\paragraph{Induction success rate.} As mentioned above, although bad data sets consume a lot of manpower and the annotation quality is relatively high, these adversarial contexts only induce unsafe responses in one generation and not multiple times. This may lead to problem that the actual induction success rate of some contexts is not high. This is also found in our measurement. More than half of the context induction success rates are actually less than 0.5 . 
\subsection{Control over Context Toxicity, Categories and Induction Success Rate}\label{3.4}
\paragraph{Control over Categories.} In order to get more diverse adversarial contexts, we control our reverse generation to augment the specified category of contexts. Intuitively, conditioning on the responses to the targeted category of contexts is easier to generate contexts belonging to the target category. We verify the conjecture on the \textit{medical} category and find that conditioning on the responses to the \textit{medical} contexts increases the proportion of \textit{medical} contexts. Furthermore, we also explore several other control methods, like prompt. This will be described in detail in \S\ref{}.
\paragraph{Control over Context Toxicity and Induction success rate.} Besides controlling the category of the generated context, we will show that we can also control the generated contexts' toxicity and induction success rate. Inspired by \citet{liu2021dexperts} and Bayes rule, we decompose the generation probability as:
\begin{equation}
    \begin{split}
    \widetilde{P}(c_t|c_{<t},r)\propto &P(c_t|c_{<t},r)(\frac{P(c_t|c_{<t},r)}{P^-(c_t|c_{<t},r)})^\alpha
    \\
    &(\frac{P(c_t|c_{<t},r)}{P(c_t|c_{<t})})^\beta
    \end{split}
\end{equation}
where $P^-$ is modeled by a toxic reverse generation model and $\alpha$ and $\beta$ are hyperparameters. The second item aims to reduce the context's toxicity and the third item aims to increase the induction success rate through Bayes rule $P(r|c)=\frac{P(c|r)P(r)}{P(c)}$. We suppose that increasing $P(r|c)$ helps improve the induction success rate of the generated context $c$. And this is proved in \S\ref{} .

==> sections/Reverse_Generation.tex <==


\section{Reverse Generation}
To automatically construct a large number of contexts with high induction success rate, we propose an effective method named reverse generation as shown in Figure \ref{fig:method}, which can directly control the factors affecting induction identified in \S\ref{3}. Concretely, we can increase the proportion of a certain category of contexts, and increase the induction success rate while reducing the toxicity of contexts. We will first introduce the basic model structure without control (\S\ref{4.1}), then describe constructing new highly inductive contexts using reverse generation with category control (\S\ref{4.2}), and finally show that reverse generation can decrease the context toxicity and increase the context's induction success rate at the same time (\S\ref{4.3}).
%An overview of the reverse generation method is shown in Figure \ref{fig:method}. % Conditioned on a response, our reverse generation module could generate relevant contexts with different control attributes.

\subsection{Basic Model Structure}
\label{4.1}
 The core idea of reverse generation is to generate a relevant context conditioned on a given response. Formally, conditioned on a response $r=(r_1,r_2,\cdots,r_M)$ with $M$ tokens, the reverse generation method learns to generate a context $c=(c_1,c_2,\cdots,c_N)$ with $N$ tokens which relates to the response. Formally, the loss function is: 
\begin{equation}\label{loss}
    \mathcal{L}=-\frac{1}{N}\sum_{t=1}^N\text{log}P(c_t|r,c_{<t}) 
\end{equation}
% The reverse generation method can control multiple attributes including category (\S\ref{4.2}), toxicity (\S\ref{4.3}), and induction success rate (\S\ref{4.3}) of the context. 


% We show the \textit{self-bleu4} metric \cite{DBLP:conf/sigir/ZhuLZGZWY18} by computing the maximum BLEU \cite{KishorePapineni2002BleuAM} of a given context against 1000 randomly sampled contexts, following \cite{perez2022red}. The \textit{distinct4} metric computes the ratio of distinct 4-grams. The \textit{toxicity} metric represents the context toxicity. The \textit{Blender/DialoGPT/Plato2 induction} represents the induction success rate for Blender/DialoGPT/Plato2. 

\begin{figure}[!t]
\includegraphics[width=\linewidth]{figs/context.pdf}% 1\linewidth
  \caption{The context distribution of the final dataset. There are 122,692 contexts in total and each category has more than 3000 diverse contexts.}
  \label{fig:context}
\end{figure}

\begin{table}[!t]
\centering
\scalebox{0.9}{
\begin{tabularx}{0.5\textwidth}{lcc}
\toprule
Method     & Initialization & \textit{Medical} ratio \\ \midrule
No control & - & 5\%  \\
Hard prompt   & - & \textbf{19\%}  \\
Soft prompt$_2$   & Random &3\%  \\
Soft prompt$_1$  & Random &9\%  \\
Soft prompt$_1$   & Vocab &10\%  \\
Soft prompt$_1$  & Hard prompt & 8\% \\
\bottomrule
\end{tabularx}}
\caption{Comparison of different controllable generation methods. Soft prompt$_2$ first fine-tunes the reverse generation model and then train the soft prompt tokens only. Soft prompt$_1$ trains the model and the soft prompt tokens together.   Different methods are trained on various kinds of contexts and we show their abilities to generate the contexts of \textit{medical} category.}
\label{tab:control}
\end{table}

\begin{table}[!t]
\centering
\scalebox{0.9}{
\begin{tabularx}{0.5\textwidth}{cccc}
\toprule
$\alpha,\beta$      & PPL & Toxicity & Induction\\ \midrule
$\alpha=0,\beta=0$ & 26.34 & 0.44 & 0.63 \\
$\alpha=2,\beta=0$ & 37.85 & 0.24 & 0.62 \\
$\alpha=0,\beta=2$ & 30.58 & 0.51 & 0.73 \\
$\alpha=2,\beta=2$ & 43.04 & 0.37 & 0.72 \\
\bottomrule
\end{tabularx}}
\caption{Comparison of different hyperparameter settings. \textit{PPL} measures the context's fluency using GPT2-large. \textit{Toxicity} measures the context's toxicity. \textit{Induction} measures the context's induction success rate.}
\label{tab:control_tox}
\end{table}

\begin{table}[!t]
\centering
\scalebox{0.9}{
\begin{tabularx}{0.5\textwidth}{lcc}
\toprule
Criteria     & Original dataset & Final dataset \\ \midrule
\# Samples & 14,302 & 122,692 \\
Self-BLEU4 & 0.25 & 0.25  \\
Distinct4   & 0.86 & 0.71 \\
Toxicity   & 0.47 &0.57  \\
Blender rate  & 0.78 &0.80  \\
DialoGPT rate   & 0.75 &0.78  \\
Plato2 rate  & 0.79 & 0.83 \\
\bottomrule
\end{tabularx}}
\caption{Comparison of the original dataset and the final dataset. \textit{\# Samples} represents the number of contexts. We show the \textit{Self-BLEU4} metric \cite{DBLP:conf/sigir/ZhuLZGZWY18} by computing the maximum BLEU \cite{KishorePapineni2002BleuAM} of a given context against 1000 randomly sampled contexts, following \cite{perez2022red}. The \textit{Distinct4} metric computes the ratio of distinct 4-grams. The \textit{Toxicity} metric represents the context toxicity. The \textit{Blender/DialoGPT/Plato2 rate} represents the induction success rate for Blender/DialoGPT/Plato2.}
\label{tab:ctx}
\end{table}

\subsection{Data Augmentation}\label{4.2}
% 包含普通增广和类别增广，类别增广方法的实验可以和类别增广那一部分一起说

\subsubsection{Generation without Control}
Considering contexts with high induction success rate are more harmful and dangerous, we focus on constructing them in our work. We first pick out the contexts with an induction success rate of no less than 50\% for all 3 dialogue models (Blender, DialoGPT and Plato2). We get 14,302 contexts from the 38,472 contexts extracted from the BAD dataset. We split the 14,302 response-context pairs into training/validation/test subsets with a ratio of 8:1:1. Then we fine-tune a reverse DialoGPT model on the training set with the loss in Equation \ref{loss}. For each of the 14,302 contexts, we randomly select one of the 10 responses from each of the 3 dialogue models to generate a context in reverse using nucleus sampling \cite{DBLP:conf/iclr/HoltzmanBDFC20} with $p=0.9$. We then pick out the contexts with an induction success rate of no less than 50\% for all 3 dialogue models and get 22,069 new contexts from $14,302\times3=42,906$ generated contexts. The comparison between the original 14,302 contexts and the augmented $14,302+22,069=36,371$ contexts is shown in Figure \ref{fig:compare_context} in the appendix. 
% We can observe that the distribution of context categories remains similar after augmentation, which suggests that our reverse generation method does not have strong preference for a specific category of contexts. 
%The diversity, toxicity and induction success rate of the contexts also remain largely unchanged after augmentation. Therefore, our simple reverse generation method can effectively construct new contexts with high induction success rate without sacrificing the contexts' diversity (in type and wording), or increasing the contexts' toxicity. 
\subsubsection{Generation with Category Control}
As shown in Figure \ref{fig:compare_context} in the appendix, the numbers of samples in some context categories are very small (e.g., the contexts of \textit{medical} category only account for 0.40\% of the total augmented contexts). This is understandable because the sample size of these categories is very small in the training set and it is harder to obtain contexts with high induction success rates in a category with a lower mean induction success rate\footnote{Most categories with a small number of contexts have relatively low induction success rates.}. Therefore, we control our reverse generation to augment the specified category of contexts. 

Intuitively, conditioning on the responses to the targeted category of contexts makes it easier to generate contexts belonging to the target category. We verify the conjecture on the \textit{medical} category. We pick up those \textit{medical} contexts and corresponding generated responses. We find that using these responses to do reverse generation can improve the proportion of \textit{medical} contexts compared with using all kinds of responses (from 0.3\% to 5\%). We thus compare abilities of several controllable methods to generate \textit{medical} contexts conditioning on the responses to the \textit{medical} contexts. We mainly consider prompt-based methods because they are simple, effective and do not sacrifice the speed of inference. We compare using hard prompt \cite{keskar2019ctrl} and soft prompt \cite{lester2021power}. We use $[category\_name]$ as our hard prompt, which is concatenated after the input response. As for soft prompt, we add 10 learnable soft tokens for each category after the input and consider different initialization strategies. As shown in Table \ref{tab:control}, using hard prompt performs best in this few-shot setting where the number of \textit{medical} contexts is small in the training set. Therefore, we use hard prompt to augment categories that include less than 3,000 contexts conditioning on the responses corresponding to the contexts of those categories. Detailed process is described in Appendix \ref{appendix:control_category}. The final augmented dataset is shown in Figure \ref{fig:context}. The context number of each category is boosted to over 3,000. We also compare the original dataset with the final dataset. As shown in Table \ref{tab:ctx}, our method largely increases the number of contexts and keeps the contexts' high induction success rate. Although the contexts' diversity decreases and the contexts' toxicity increases to some extent, they are still within an acceptable range.


\subsection{Control of Context Toxicity and Induction Success Rate}\label{4.3}

Although we can see in Figure \ref{fig:induce_rate} that the context with higher toxicity usually has a higher induction success rate, the adversarial context with lower toxicity is more difficult to be detected by the classifier, which is more difficult to be defended and more harmful. Therefore, we explore control reverse generation to decrease the context toxicity and increase the context's induction success rate at the same time. In this way, we can get more harmful adversarial contexts with low toxicity and high induction success rate. Inspired by \citet{liu2021dexperts} and Bayes' rule, we decompose the generation probability as:
\begin{equation}
    \begin{split}
    \widetilde{P}(c_t|c_{<t},r)\propto &P(c_t|c_{<t},r)(\frac{P(c_t|c_{<t},r)}{P^-(c_t|c_{<t},r)})^\alpha
    \\
    &(\frac{P(c_t|c_{<t},r)}{P(c_t|c_{<t})})^\beta
    \end{split}
\end{equation}
where $P^-$ is modeled by a toxic reverse generation model and $\alpha$ and $\beta$ are hyperparameters. The second item aims to reduce the context's toxicity and the third item aims to increase the induction success rate through Bayes rule $P(r|c)=\frac{P(c|r)P(r)}{P(c)}$. We suppose that increasing $P(r|c)$ helps improve the induction success rate of the generated context $c$. We fine-tune DialoGPT on the training set of the filtered BAD dataset and compare different hyperparameters on the test set. The toxic reverse generation model is trained on the subset where each context's toxicity is larger than 0.5. 
As shown in Table \ref{tab:control_tox}, with $\alpha=2 $ and $\beta=2$, we could simultaneously reduce the context's toxicity and increase the context's induction success rate while keeping the context's fluency acceptable, which suggests the effectiveness of our controllable generation method. Note that we didn't control the context's toxicity and induction success rate during data augmentation because we hope our dataset could have diverse contexts with different toxicities and induction success rates. But the method is useful for specifically constructing contexts with low toxicities and high induction success rates.
